Planning for Learning Object Properties

Autonomous agents embedded in a physical environment need the ability to recognize objects and their properties from sensory data. Such a perceptual ability is often implemented by supervised machine learning models, which are pre-trained using a set of labelled data. In real-world, open-ended deployments, however, it is unrealistic to assume to have a pre-trained model for all possible environments. Therefore, agents need to dynamically learn/adapt/extend their perceptual abilities online, in an autonomous way, by exploring and interacting with the environment where they operate. This paper describes a way to do so, by exploiting symbolic planning. Specifically, we formalize the problem of automatically training a neural network to recognize object properties as a symbolic planning problem (using PDDL). We use planning techniques to produce a strategy for automating the training dataset creation and the learning process. Finally, we provide an experimental evaluation in both a simulated and a real environment, which shows that the proposed approach is able to successfully learn how to recognize new object properties.

==> algorithms/main_algorithm.tex <==


\begin{algorithm}[t]
\caption{Algorithm: \textcolor{red}{version 1: with low level actions}}
\label{alg:algorithm}
\textbf{Input}: $\planprob$, $p$, $\rho_{od}$, $\rho_{\P}$ and $\textsc{maxObs}\in\mathbb{N}$.
% \\ \textbf{Output}: $\D_{p}$

\begin{algorithmic}[1] %[1] enables line numbers


\STATE $\planprob' \gets \textsc{planLearnProblem}(\planprob, p)$ \label{algline:init_plan_prob}

\STATE $\D_{p} \gets \langle\emptyset,\emptyset\rangle$  \label{algline:init_D}

\STATE $s \gets s_0'$ \label{algline:init_s}

\WHILE {$|\D_p| < \textsc{maxObs}$}
    
    \STATE $\pi\gets\textsc{plan}(\planprob)$ \label{algline:plan}
    
    \IF{$\pi = \textsc{None}$}
    
        \STATE $\bo \gets \textsc{explore}()$ \label{algline:explore}
    
    \ELSE
    
        \STATE $op(\bc)\gets\textsc{pop}(\pi)$ \label{algline:pop-plan}
        
        \STATE $\bo \gets \textsc{compile}(op(\bc))$ \label{algline:compile-plan}
    
    \ENDIF
    
    \STATE $o \gets$\textsc{pop}$(\bo)$ \label{algline:pop-operation}
    
    \STATE $success\gets \textsc{Execute}(o)$ \label{algline:exec}
    
    \STATE $x\gets \textsc{Perceive}()$ \label{algline:perceive}
    
    % \STATE $\C_{\bx}\gets \textsc{detectObjects}(\bx)$
    \STATE $\C_{x}, \T'(\C_x)\gets \rho_{od}(x)$
    
    \STATE $\P'(\C_{x})\gets \rho_{\P}(x, \T'(\C_{x}))$ \label{algline:map-perception-predicates}
    
    \STATE $s \gets s \cup \P'(\C_{x}) \cup \T'(\C_{x})$ \label{algline:update-state}
    
    \STATE $\C' \gets \C' \cup \C_x$ \label{algline:map-perception-objects}
    
    \IF{$\pi {\not=}$ \textsc{None} \textbf{and} $success$ \textbf{and} $|\bo| == 0$} \label{algline:check-action-success}
    
        \STATE $s \gets s \cup \eff^+(op(\bc)) \setminus \eff^-(op(\bc))$ \label{algline:update-state-effects}
    
    \ENDIF
    
    \STATE $y \gets \{p(c)\mid \texttt{known}(c,p)\in s,\;c\in \C_{x}\}$ \label{algline:get-obs-labels}
    
    \IF{$y {\not=} \emptyset$ }
    
        \STATE $\D_{p} \gets \textsc{append}(\D_{p}, \langle x, y\rangle)$ \label{algline:update-dataset}
    
    \ENDIF

\ENDWHILE \label{algline:end-while}

\RETURN $\D_{p}$ \label{algline:end_return}

\end{algorithmic}

\end{algorithm}

==> algorithms/main_algorithm_2.tex <==


\begin{algorithm}[t]
\caption{Algorithm: \textcolor{red}{version 2: without low level actions}}
\label{alg:algorithm}
\textbf{Input}: $\actmodel$, $p$, $\T\subset\P$, $\rho_{od}$, $\rho_{\P}$ and $\textsc{maxIter}\in\mathbb{N}$.
% \\ \textbf{Output}: $\D_{p}$

\begin{algorithmic}[1] %[1] enables line numbers


\STATE $\planprob' \gets \textsc{planLearnProblem}(\actmodel, p, \T)$ \label{algline:init_plan_prob}

\STATE $\D_{p} \gets \langle\emptyset,\emptyset\rangle$  \label{algline:init_D}

\STATE $s \gets s_0'$ \label{algline:init_s}

% \WHILE {$|\D_p| < \textsc{maxObs}$}
\FOR {$i = 1 \textbf{ to } \textsc{maxIter}$}
    
    \IF{$g \models s$ }
        \STATE \textbf{break}
    \ENDIF
    
    \STATE $\pi\gets\textsc{plan}(\planprob')$ \label{algline:plan}
    
    \IF{$\pi = \textsc{None}$}
    
        \STATE $op \gets \textsc{explore}()$ \label{algline:explore}
    
    \ELSE
    
        \STATE $op\gets\textsc{pop}(\pi)$ \label{algline:pop-plan}
        
        % \STATE $\bo \gets \textsc{compile}(op(\bc))$ \label{algline:compile-plan}
    
    \ENDIF
    
    % \STATE $op(\bc) \gets$\textsc{pop}$(\pi)$ \label{algline:pop-operation}
    
    \STATE $success\gets \textsc{Execute}(op)$ \label{algline:exec}
    
    \STATE $x\gets \textsc{Perceive}()$ \label{algline:perceive}
    
    % \STATE $\C_{x}, \T'(\C_x)\gets \rho_{od}(x)$
    
    % \STATE $\P'(\C_{x})\gets \rho_{\P}(x, \T'(\C_{x}))$ \label{algline:map-perception-predicates}
    
    % \STATE $s \gets s \cup \P'(\C_{x}) \cup \T'(\C_{x})$ \label{algline:update-state}
    
    \STATE $s, \C_x \gets \textsc{updateState}(s, x, \rho_{od}, \rho_{\P})$ \label{algline:update-state}

    % \STATE $\C' \gets \C' \cup \C_x$ \label{algline:map-perception-objects}
    
        
    \IF{$\pi {\not=}$ \textsc{None} \textbf{and} $success$} \label{algline:check-action-success}
    
        \STATE $s \gets s \cup \eff^+(op) \setminus \eff^-(op)$ \label{algline:update-state-effects}
    
    \ENDIF
    
    \STATE $y \gets \{p\mid \texttt{known}(o,p)\in s,\;o\in \C_{x}\}$ \label{algline:get-obs-labels}
    
    \IF{$y {\not=} \emptyset$ }
    
        \STATE $\D_{p} \gets \textsc{append}(\D_{p}, \langle x, y\rangle)$ \label{algline:update-dataset}
    
    \ENDIF

% \ENDWHILE \label{algline:end-while}
\ENDFOR \label{algline:end-for}

% \RETURN $\D_{p}$ \label{algline:end_return}

\end{algorithmic}

\end{algorithm}

==> figures/obs_action_schema.tex <==
         

\begin{myverbbox}{\obsactionschema}
(:action obs
  :parameters (?o ?p)
  :precondition (and (has_property ?o ?p) 
                     (known ?o ?p))
  :effect (observed ?o ?p))
\end{myverbbox}


\begin{tikzpicture} 
    
    \node (obs_action_schema) [scale=.6,fill=green!30, draw, rectangle, anchor=east, label=Initial state]{\obsactionschema}; 

\end{tikzpicture}

==> sections/01_introduction_new.tex <==
\section{Introduction}

Agents embedded in a physical environment, like autonomous robots,
need the ability to perceive objects in the environment and recognise
their properties. For instance, a robot operating in an apartment
should be able to recognize whether a certain door is open or closed,
a cup is full (of coffee) or empty, the TV is on or off, and so on.
%
The capability of abstracting the perceptions (usually continuous data)
into a symbolic state enables the agent to adopt symbolic reasoning methods 
such as automated planning to produce strategies for reaching complex goals. 

The common machine learning approach to provide an agent with such
perceptual capabilities consists in pre-training a (set of) perception
models from data sets that contain hundreds of thousands of
semantically annotated images. \cite{}

However, this offline training approach
is in stark contrast with a main requirement in several robotics
applications, where it is widely recognized that perception is an
active and exploratory process based on visual exploration rather than
on the analysis of static images. This is also confirmed by the
emerging popular research area of interactive perception
\cite{bohg2017}.

Indeed, agents embedded in real-world, open-ended environments should be able to dynamically and autonomously improve their perceptual abilities by exploring and executing actions in the environment.
%
In the case of supervised deep learning approaches, an open and interesting challenge is whether they can train autonomously and online their learning model, e.g., by collecting autonomously the needed training data to learn object properties.
By itself this can be seen as a planning proble, i.e., the agent has to \emph{plan 
to learn/improve a certain perceptual capability}.

In this paper, we explore a way to automatically collect the right data for training online a neural network able to recognize properties of objects that are perceived in the environment. We devise an approach based on automated planning for deciding what training data to collect and how to train neural networks. According to this idea we provide the following contributions.

\begin{itemize}
\item 
We formalize the problem of automatically training a neural net to predict object properties  as a planning problem. The planning domain contains actions that can change the properties of objects (e.g., opening a book) and observation actions (e.g., observe the open book) that can be used to train neural networks for recognizing object properties. The planning problem is formalized with goals that represent the objective to discover objects in the environment and learn how to recognize their properties.
\item
Given the planning problem, we implement it in PDDL \cite{McDermott:98-PDDL} and use planning techniques to automatize the training and learning process.
The planning algorithm automatically maps low level perceptions (e.g., images of an open book) into symbolic properties of objects at the planning level (e.g., "the book is open" in PDDL).  
\item
We provide an experimental evaluation both in a realistic simulated environment \cite{ai2thor}, and in a real world setting. In the simulated environment, we evaluate the ability to learn certain object properties (e.g., open, toggle, fill, dirty), under two different conditions of object detection (noisy and ground truth). The results indicate that the approach is able to successfully learn and recognize the object properties with high precision/recall for most object classes. In the real world experiment, actions for changing object properties (e.g., opening a book) are performed in a cooperative way with humans, i.e., by interacting with humans and asking them to physically perform the required action.
\end{itemize}

The paper is structured as follows, .... [[TO BE REVISED]] in Section \ref{sec:preliminaries} we formalize some fundamentals of symbolic planning and define the problem addressed in this paper. In Section \ref{sec:method}, we formally define our approach and describe it in detail together with our solution proposal. Afterwards, in Section \ref{sec:experiments} we evaluate the performance of the proposed approach where a robotic agent learns to recognize new relationships by interacting with objects in photo-realistic simulated environments. Finally, in Section \ref{sec:relatedwork} we analyze the literature about the integration of planning and learning, planning from continuous observations, and learning through interaction with the environment.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/01_introduction_paolo.tex <==
\section{Introduction}

Agents embedded in a physical environment, like autonomous robots, need the ability to perceive objects in the environment and recognise their properties. For instance, a robot operating in an indoor environment should be able to recognize whether a book found in the environment is open or closed, a cup is full (of coffee) or empty, the TV is on or off, a mirror is clean or dirty, and so on.

The common machine vision approach is to provide an agent with such perceptual capabilities by pre-training learning models from data sets that contain hundreds of thousands of semantic annotated static images, e.g., through 
supervised deep learning neural nets that can be then used by the robot to recognize object properties.

However, this offline ``pre-training" approach is in stark contrast with a main requirement in several robotics applications, where it is widely recognized that perception for robots is an active and exploratory process based on visual exploration rather than on the analysis of static images, as shown in the works in an emerging and now popular research area, interactive perception \cite{bohg2017}. 

Indeed, agents embedded in real-world, open-ended environments should be able to dynamically and autonomously enrich their perceptual abilities by exploring the environment.
%
In the case of supervised deep learning approaches, an open and interesting challenge is whether they can train autonomously and online their learning model, e.g., by collecting autonomously the needed training data to learn object properties.


In this paper, we explore a way to automatically collect the right data for training online a neural network able to recognize properties of objects that are perceived in the environment. We devise an approach based on automated planning for deciding what training data to collect and how to train neural networks. According to this idea we provide the following contributions.

\begin{itemize}
\item 
We formalize the problem of automatically training a neural net as a planning problem, thus providing a principled way for integrating planning with the training of learning-based perception models. The planning domain contains actions that can change the properties of objects (e.g., opening a book) and observation actions (e.g. observe the open book) that can be used to train neural networks for recognizing object properties. The planning problem is formalized with goals that represent the objective to discover objects in the environment and learn how to recognize their properties.
\item
Given the planning problem, we implement it in PDDL \cite{McDermott:98-PDDL} and use planning techniques to automatize the training and learning process.
The planning algorithm automatically maps low level perceptions (e.g., images of an open book) into symbolic properties of objects at the planning level (e.g., "the book is open" in PDDL).  
\item
We provide an experimental evaluation both in a realistic simulated environment \cite{ai2thor}, and in a real world setting. In the simulated environment, we evaluate the ability to learn certain object properties (e.g., open, toggle, fill, dirty), under two different conditions of object detection (noisy and ground truth). The results indicate that the approach is able to successfully learn and recognize the object properties with high precision/recall for most object classes. In the real world experiment, actions for changing object properties (e.g., opening a book) are performed in a cooperative way with humans, i.e., by interacting with humans and asking them to physically perform the required action.
\end{itemize}

The paper is structured as follows, .... [[TO BE REVISED]] in Section \ref{sec:preliminaries} we formalize some fundamentals of symbolic planning and define the problem addressed in this paper. In Section \ref{sec:method}, we formally define our approach and describe it in detail together with our solution proposal. Afterwards, in Section \ref{sec:experiments} we evaluate the performance of the proposed approach where a robotic agent learns to recognize new relationships by interacting with objects in photo-realistic simulated environments. Finally, in Section \ref{sec:relatedwork} we analyze the literature about the integration of planning and learning, planning from continuous observations, and learning through interaction with the environment.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/PepperMetricsOLD.tex <==

%bowl: Prec 0.63   Recall 0.98 Fscore 0.77
%laptop  Acc 0.99    Prec 0.97   Recall 1.00 Fscore 0.99
%book Acc 0.99    Prec 1.00   Recall 0.99 Fscore 0.99
%Cup Acc 0.88	Prec 0.93	Recall 0.83	Fscore 0.88

\begin{table}[t]
\centering
\small
%\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|lllll}
\toprule
    &   Bowl & Laptop & Book & Cup & weight avg\\ \midrule
  P. & 0.63 & 0.97 & 1.00 & 0.93 & 0.88  \\
  R. & 0.98 & 1.00 & 0.99 & 0.83 & 0.95\\
\bottomrule
\end{tabular}
%}
\caption{Precision and recall obtained by the neural network predicting the truth value of the object properties.}
\label{tab:PepperMetrics}
\end{table}
% \begin{table}[t]
% \centering
% \small
% %\resizebox{0.5\textwidth}{!}{
% \begin{tabular}{ll|l}
% \toprule

%  Object type &    \textsf{P} &    \textsf{R}  \\
% \midrule
%        bowl &       0.63 &         0.98     \\
%        laptop &       0.97 &         1.00     \\
%        book &       1.00 &         0.99     \\
%       \hline\hline
%  Weighted avg &        0.87 &           0.99              \\
% \bottomrule
% \end{tabular}
% %}
% \caption{Precision and recall obtained by the neural network predicting the truth value of the object properties.}
% \label{tab:PepperMetrics}
% \end{table}


==> tables/dirty_metrics.tex <==
\begin{table*}
\centering
\caption{Performance of precision, recall and f-measure obtained with the neural network associated to the dirty relationship.}
\label{tab:dirty_metrics}
\resizebox{\textwidth}{!}{
\begin{tabular}{lllll|llll|llll|llll|llll}
\toprule
& \multicolumn{4}{c|}{$F$}  &  \multicolumn{4}{c|}{$P$} &  \multicolumn{4}{c|}{$R$}&  \multicolumn{4}{c|}{$Train$}&  \multicolumn{4}{c}{$Test$}  \\
 Object type &    V1 &    V2 &    V3 &    V4 &    V1 &    V2 &    V3 &    V4 &    V1 &    V2 &    V3 &    V4 &   V1 &   V2 &    V3 &    V4 &  V1 &  V2 &  V3 &  V4 \\
\midrule
         bed &  0.56 &  0.55 &  0.49 &  0.69 &  0.95 &  0.57 &  0.94 &  0.67 &  0.43 &  0.61 &  0.37 &  0.78 & 1502 &  671 &  4520 &  2188 & 564 & 564 & 564 & 564 \\
        bowl &  0.71 &  0.81 &  0.62 &  0.82 &  0.67 &  0.98 &  0.83 &  0.94 &  0.81 &  0.73 &   0.6 &  0.78 &  383 & 1027 &  1992 &  4024 & 280 & 216 & 280 & 280 \\
       cloth &  0.83 &  0.78 &  0.65 &  0.81 &  0.93 &  0.95 &  0.68 &     1 &  0.78 &   0.7 &  0.62 &  0.72 &   61 &  503 &   112 &  1196 &  96 & 210 & 210 & 210 \\
         cup &  0.75 &  0.64 &  0.65 &  0.75 &  0.63 &  0.99 &  0.55 &  0.97 &  0.95 &  0.54 &  0.81 &  0.65 &  146 &  986 &   150 &  3159 &  96 & 262 & 262 & 262 \\
      mirror &  0.75 &  0.84 &  0.79 &  0.87 &  0.91 &   0.9 &  0.83 &     1 &  0.68 &   0.8 &  0.76 &  0.81 & 2490 & 3100 & 13987 & 20958 & 654 & 678 & 678 & 678 \\
         mug &  0.42 &  0.81 &  0.77 &  0.76 &  0.88 &  0.94 &   0.8 &  0.94 &  0.42 &  0.74 &  0.78 &  0.67 &  225 & 1367 &  1266 &  6054 & 230 & 432 & 432 & 432 \\
         pan &   0.8 &  0.87 &  0.76 &  0.93 &  0.76 &  0.99 &  0.65 &     1 &  0.87 &  0.79 &  0.95 &  0.87 &   20 &  476 &    79 &  1259 & 140 & 200 & 200 & 200 \\
       plate &  0.75 &  0.85 &  0.76 &  0.88 &  0.61 &  0.97 &  0.64 &  0.97 &  0.97 &  0.77 &  0.96 &  0.81 &   47 & 1304 &   187 &  6146 & 166 & 406 & 406 & 406 \\
         pot &   0.8 &  0.99 &  0.76 &  0.93 &  0.76 &  0.99 &  0.68 &  0.99 &  0.91 &  0.98 &  0.92 &  0.89 &   51 &  929 &    74 &  2509 & 210 & 272 & 272 & 272 \\
       \hline\hline
Weighted avg &  0.68 &  0.78 &  0.69 &  0.82 &  0.84 &  0.89 &  0.77 &  0.92 &  0.68 &  0.74 &  0.73 &  0.78 &    - &    - &     - &     - &   - &   - &   - &   - \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/dirty_metrics_learning.tex <==
\begin{table}[t]
\centering


\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lll|ll|ll|ll}
\toprule
& \multicolumn{2}{c|}{$Test$}  &  \multicolumn{2}{c|}{$Train$} &  \multicolumn{2}{c|}{$P$}&  \multicolumn{2}{c}{$R$}\\
 Object type &    \textsf{ND} &    \textsf{GTD} &  \textsf{ND} &    \textsf{GTD} &  \textsf{ND} &    \textsf{GTD} &   \textsf{ND} &   \textsf{GTD}\\
\midrule
         bed &      564 &         564 &     1502 &         671 &          0.95 &        0.57 &       0.43 &        0.61 \\
        bowl &      280 &         280 &      383 &        1027 &          0.67 &        0.98 &       0.81 &        0.73 \\
       cloth &       96 &         210 &       61 &         503 &          0.93 &        0.95 &       0.78 &         0.7 \\
         cup &       96 &         262 &      146 &         986 &          0.63 &        0.99 &       0.95 &        0.54 \\
      mirror &      654 &         678 &     2490 &        3100 &          0.91 &         0.9 &       0.68 &         0.8 \\
         mug &      230 &         432 &      225 &        1367 &          0.88 &        0.94 &       0.42 &        0.74 \\
         pan &      140 &         200 &       20 &         476 &          0.76 &        0.99 &       0.87 &        0.79 \\
       plate &      166 &         406 &       47 &        1304 &          0.61 &        0.97 &       0.97 &        0.77 \\
         pot &      210 &         272 &       51 &         929 &          0.76 &        0.99 &       0.91 &        0.98 \\
         \hline \hline
Weighted avg &        - &           - &        - &           - &          0.84 &        0.89 &       0.68 &        0.74 \\
\bottomrule
\end{tabular}
}
\caption{Size of the test set (columns 2-3) and generated training set (columns 4-5), precision (columns 6-7) and recall (columns 8-9) obtained by the neural network predicting the \textsc{dirty} property. The weighted average (last line) uses the number of test observations as weights.}
\label{tab:dirty_metrics_learning}
\end{table}


==> tables/extended_action_schema.tex <==

\begin{table}[t]
  \centering
%   \begin{tabular}{clp{1.5cm}ll}
\scriptsize
  \begin{tabular}{p{0.5cm}p{1cm}p{2.4cm}p{2.1cm}p{0.3cm}}
    \multicolumn{1}{c}{$op$} & \multicolumn{1}{c}{$\param{(op)}$} & \multicolumn{1}{c}{$\prec{(op)}$} & \multicolumn{1}{c}{$\eff^+{(op)}$} & \multicolumn{1}{c}{$\eff^-{(op)}$} \\ \hline 
    $\texttt{obs}$ & $o, \name{t}, \name{p}$ & $\texttt{has\_property}(o, \name{p}), $ $\lnot\texttt{viewed}(o, \name{p})$, $\texttt{known}(o, \name{p})$, $\texttt{property}(\name{p})$ $\texttt{type}(o)$ & $\texttt{observed}(\name{t}, \name{p})$, $\texttt{viewed}(o, \name{p})$ & $\emptyset$\\
    $\texttt{learn}$ & $o, \name{t}, \name{p}$ & $\texttt{observed}(o, \name{t}), $ $\texttt{observed}(o, \name{p})$, $\texttt{property}(\name{t})$, $\texttt{property}(\name{p})$, $\texttt{type}(o)$ & $\texttt{learned}(o, \name{t}, \name{p})$ & $\emptyset$\\\hline
  \end{tabular}
  \caption{Action schema of the operators \code{obs} and \code{learn}.}
  \label{tab:extended_action_schema}
\end{table}




% \begin{table}[t]
%   \centering
% %   \begin{tabular}{clp{1.5cm}ll}
% \scriptsize
%   \begin{tabular}{p{0.5cm}p{1cm}p{2.4cm}p{2.1cm}p{0.3cm}}
%     \multicolumn{1}{c}{$op$} & \multicolumn{1}{c}{$\param{(op)}$} & \multicolumn{1}{c}{$\prec{(op)}$} & \multicolumn{1}{c}{$\eff^+{(op)}$} & \multicolumn{1}{c}{$\eff^-{(op)}$} \\ \hline 
%     $\code{obs}$ & $o, \name{t}, \name{p}$ & $\code{has\_property}(o, \name{p}), $ $\lnot\code{viewed}(o, \name{p})$, $\code{known}(o, \name{p})$, $\code{property}(\name{p})$ $\code{type}(o)$ & $\code{observed}(\name{t}, \name{p})$, $\code{viewed}(o, \name{p})$ & $\emptyset$\\
%     $\code{learn}$ & $o, \name{t}, \name{p}$ & $\code{observed}(o, \name{t}), $ $\code{observed}(o, \name{p})$, $\code{property}(\name{t})$, $\code{property}(\name{p})$, $\code{type}(o)$ & $\code{learned}(o, \name{t}, \name{p})$ & $\emptyset$\\\hline
%   \end{tabular}
%   \caption{Action schema of the operators \code{obs} and \code{learn}.}
%   \label{tab:extended_action_schema}
% \end{table}

==> tables/fill_metrics.tex <==
\begin{table*}
\centering
\caption{Performance of precision, recall and f-measure obtained with the neural network associated to the fill relationship.}
\label{tab:fill_metrics}
\resizebox{\textwidth}{!}{
\begin{tabular}{lllll|llll|llll|llll|llll}
\toprule
& \multicolumn{4}{c|}{$F$}  &  \multicolumn{4}{c|}{$P$} &  \multicolumn{4}{c|}{$R$}&  \multicolumn{4}{c|}{$Train$}&  \multicolumn{4}{c}{$Test$}  \\
 Object type &    V1 &    V2 &    V3 &    V4 &    V1 &    V2 &    V3 &    V4 &    V1 &    V2 &    V3 &    V4 &  V1 &   V2 &   V3 &   V4 &  V1 &  V2 &  V3 &  V4 \\
\midrule
      bottle &  0.79 &     0 &   0.9 &  0.95 &  0.65 &     0 &     1 &     1 &     1 &     0 &  0.82 &  0.91 &  78 &  150 &   78 &  150 &  22 &  22 &  22 &  22 \\
        bowl &  0.64 &  0.86 &  0.73 &   0.9 &  0.64 &     1 &  0.86 &     1 &  0.73 &  0.77 &  0.74 &  0.84 & 390 & 1091 & 1562 & 4665 & 328 & 256 & 328 & 328 \\
         cup &  0.65 &  0.71 &  0.55 &  0.71 &  0.92 &   0.9 &  0.77 &   0.9 &  0.56 &  0.68 &  0.64 &  0.68 & 200 & 1028 &  328 & 3485 & 116 & 286 & 286 & 286 \\
  houseplant &  0.56 &  0.62 &  0.37 &  0.11 &   0.5 &   0.5 &   0.5 &   0.5 &  0.65 &  0.82 &  0.32 &  0.07 &  18 &   72 &   54 &  216 &  34 &  34 & 128 & 128 \\
      kettle &   - &  0.31 &   - &  0.06 &   - &  0.25 &   - &  0.25 &   - &   0.4 &   - &  0.03 & - &  337 &  - &  518 & - &  84 & - &  84 \\
         mug &  0.59 &  0.62 &  0.63 &  0.59 &   0.8 &  0.86 &  0.84 &  0.82 &  0.51 &  0.56 &  0.52 &  0.51 & 250 & 1136 & 1598 & 4701 & 126 & 354 & 412 & 412 \\
         pot &  0.72 &  0.87 &  0.72 &  0.88 &  0.67 &     1 &  0.61 &     1 &  0.89 &  0.79 &  0.94 &  0.81 &  93 &  809 &  297 & 2221 & 226 & 274 & 274 & 274 \\
       \hline\hline
Weighted avg &  0.66 &  0.71 &  0.63 &  0.67 &   0.7 &  0.86 &  0.76 &  0.85 &  0.72 &  0.66 &  0.66 &  0.61 &   - &    - &    - &    - &   - &   - &   - &   - \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/fill_metrics_learning.tex <==
\begin{table}[t]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lll|ll|ll|ll}
\toprule
& \multicolumn{2}{c|}{$Test$}  &  \multicolumn{2}{c|}{$Train$} &  \multicolumn{2}{c|}{$P$}&  \multicolumn{2}{c}{$R$}\\
 Object type &    \textsf{ND} &    \textsf{GTD} &  \textsf{ND} &    \textsf{GTD} &  \textsf{ND} &    \textsf{GTD} &   \textsf{ND} &   \textsf{GTD}\\
\midrule
      bottle &       22 &          22 &       78 &         150 &          0.65 &           0 &          1 &           0 \\
        bowl &      328 &         256 &      390 &        1091 &          0.64 &           1 &       0.73 &        0.77 \\
         cup &      116 &         286 &      200 &        1028 &          0.92 &         0.9 &       0.56 &        0.68 \\
  houseplant &       34 &          34 &       18 &          72 &           0.5 &         0.5 &       0.65 &        0.82 \\
      kettle &      - &          84 &      - &         337 &           - &        0.25 &        - &         0.4 \\
         mug &      126 &         354 &      250 &        1136 &           0.8 &        0.86 &       0.51 &        0.56 \\
         pot &      226 &         274 &       93 &         809 &          0.67 &           1 &       0.89 &        0.79 \\
      \hline\hline
Weighted avg &        - &           - &        - &           - &           0.7 &        0.86 &       0.72 &        0.66 \\
\bottomrule
\end{tabular}
}
\caption{Size of the test set (columns 2-3) and generated training set (columns 4-5), precision (columns 6-7) and recall (columns 8-9) obtained by the neural network predicting the \textsc{fill} property. The weighted average (last line) uses the number of test observations as weights.}
\label{tab:fill_metrics_learning}
\end{table}


==> tables/open_metrics.tex <==
\begin{table*}
% \setlength{\tabcolsep}{2pt}
\centering
\caption{Performance of precision, recall and f-measure obtained with the neural network associated to the open relationship.}
\label{tab:open_metrics}
\resizebox{\textwidth}{!}{
\begin{tabular}{lllll|llll|llll|llll|llll}
\toprule
& \multicolumn{4}{c|}{$F$}  &  \multicolumn{4}{c|}{$P$} &  \multicolumn{4}{c|}{$R$}&  \multicolumn{4}{c|}{$Train$}&  \multicolumn{4}{c}{$Test$}  \\
  Object type &    V1 &    V2 &    V3 &    V4 &    V1 &    V2 &    V3 &    V4 &    V1 &    V2 &    V3 &    V4 &   V1 &   V2 &   V3 &    V4 &   V1 &   V2 &   V3 &   V4 \\
\midrule
         book &  0.86 &  0.86 &  0.67 &  0.87 &     1 &  0.94 &  0.96 &  0.95 &  0.76 &  0.81 &  0.55 &  0.82 &  367 & 1471 & 1120 &  5578 &  148 &  268 &  180 &  268 \\
          box &   0.5 &  0.63 &   0.7 &  0.66 &  0.92 &  0.88 &  0.92 &  0.86 &  0.37 &  0.54 &  0.58 &  0.58 &  959 & 1044 & 3293 &  3710 &  204 &  204 &  244 &  244 \\
      cabinet &  0.73 &  0.75 &  0.76 &  0.84 &  0.81 &   0.8 &  0.89 &  0.86 &  0.74 &  0.79 &  0.72 &  0.82 & 1545 & 1669 & 6556 &  6864 & 2892 & 2892 & 2892 & 2892 \\
       drawer &  0.75 &  0.69 &  0.75 &  0.75 &  0.79 &  0.75 &  0.84 &  0.83 &  0.77 &  0.71 &   0.7 &  0.73 & 1237 & 2624 & 9358 & 24244 & 3343 & 3747 & 3803 & 3803 \\
       fridge &  0.73 &   0.7 &  0.66 &  0.75 &  0.78 &  0.81 &  0.68 &  0.75 &  0.72 &  0.75 &  0.67 &   0.8 &  803 & 1109 & 2114 &  2792 &  400 &  400 &  400 &  400 \\
       kettle &   - &     0 &   - &  0.26 &   - &     0 &   - &   0.5 &   - &     0 &   - &  0.17 &  - &  137 &  - &   274 &  - &   34 &  - &   70 \\
       laptop &  0.87 &  0.88 &  0.68 &  0.81 &  0.93 &  0.97 &  0.85 &  0.96 &  0.85 &  0.82 &  0.61 &  0.75 & 1124 & 1531 & 4338 &  6648 &  360 &  360 &  396 &  396 \\
    microwave &  0.58 &  0.71 &  0.57 &  0.69 &  0.68 &  0.82 &     1 &  0.89 &   0.5 &  0.68 &  0.44 &   0.6 &  742 &  843 & 2719 &  2707 &  250 &  250 &  250 &  250 \\
showercurtain &  0.44 &  0.85 &  0.76 &  0.79 &  0.47 &  0.96 &  0.83 &  0.75 &  0.41 &  0.76 &  0.72 &  0.87 &  271 &  567 &  710 &  1097 &  144 &  134 &  206 &  206 \\
   showerdoor &  0.31 &   0.8 &  0.44 &  0.83 &  0.88 &  0.71 &  0.75 &  0.77 &  0.19 &  0.98 &  0.56 &  0.95 &   56 &  346 &  112 &   581 &   74 &  140 &  140 &  140 \\
       toilet &  0.65 &  0.76 &  0.86 &  0.78 &  0.89 &   0.9 &   0.9 &  0.87 &  0.63 &  0.74 &  0.83 &   0.8 & 1024 & 1148 & 2987 &  3159 &  356 &  356 &  356 &  356 \\
       
       \hline\hline
 Weighted avg &  0.72 &  0.73 &  0.74 &  0.78 &  0.81 &  0.79 &  0.86 &  0.84 &  0.72 &  0.74 &  0.69 &  0.76 &    - &    - &    - &     - &    - &    - &    - &    - \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/open_metrics_learning.tex <==
\begin{table}[t]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lll|ll|ll|ll}
\toprule
& \multicolumn{2}{c|}{$Test$}  &  \multicolumn{2}{c|}{$Train$} &  \multicolumn{2}{c|}{$P$}&  \multicolumn{2}{c}{$R$}\\
 Object type &    \textsf{ND} &    \textsf{GTD} &  \textsf{ND} &    \textsf{GTD} &  \textsf{ND} &    \textsf{GTD} &   \textsf{ND} &   \textsf{GTD}\\
\midrule
         book &      148 &         268 &      367 &        1471 &             1 &        0.94 &       0.76 &        0.81 \\
          box &      204 &         204 &      959 &        1044 &          0.92 &        0.88 &       0.37 &        0.54 \\
      cabinet &     2892 &        2892 &     1545 &        1669 &          0.81 &         0.8 &       0.74 &        0.79 \\
       drawer &     3343 &        3747 &     1237 &        2624 &          0.79 &        0.75 &       0.77 &        0.71 \\
       fridge &      400 &         400 &      803 &        1109 &          0.78 &        0.81 &       0.72 &        0.75 \\
       laptop &      360 &         360 &     1124 &        1531 &          0.93 &        0.97 &       0.85 &        0.82 \\
    microwave &      250 &         250 &      742 &         843 &          0.68 &        0.82 &        0.5 &        0.68 \\
showercurtain &      144 &         134 &      271 &         567 &          0.47 &        0.96 &       0.41 &        0.76 \\
   showerdoor &       74 &         140 &       56 &         346 &          0.88 &        0.71 &       0.19 &        0.98 \\
       toilet &      356 &         356 &     1024 &        1148 &          0.89 &         0.9 &       0.63 &        0.74 \\
      \hline\hline
 Weighted avg &        - &           - &        - &           - &          0.81 &         0.8 &       0.72 &        0.75 \\
\bottomrule
\end{tabular}
}
\caption{Size of the test set (columns 2-3) and generated training set (columns 4-5), precision (columns 6-7) and recall (columns 8-9) obtained by the neural network predicting the \textsc{open} property. The weighted average (last line) uses the number of test observations as weights.}
\label{tab:open_metrics_learning}
\end{table}


==> tables/toggle_metrics.tex <==
\begin{table*}
\centering
\caption{Performance of precision, recall and f-measure obtained with the neural network associated to the toggle relationship.}
\label{tab:toggle_metrics}
\resizebox{\textwidth}{!}{
\begin{tabular}{lllll|llll|llll|llll|llll}
\toprule
& \multicolumn{4}{c|}{$F$}  &  \multicolumn{4}{c|}{$P$} &  \multicolumn{4}{c|}{$R$}&  \multicolumn{4}{c|}{$Train$}&  \multicolumn{4}{c}{$Test$}  \\
  Object type &    V1 &    V2 &    V3 &    V4 &    V1 &    V2 &    V3 &    V4 &    V1 &    V2 &    V3 &    V4 &   V1 &   V2 &   V3 &   V4 &  V1 &  V2 &  V3 &  V4 \\
\midrule
       candle &  0.61 &  0.42 &  0.49 &  0.24 &  0.59 &  0.33 &  0.51 &  0.45 &  0.63 &   0.6 &  0.52 &  0.28 &    3 &  118 &    9 &  545 &  54 & 124 & 144 & 284 \\
    cellphone &  0.83 &  0.86 &  0.63 &  0.94 &  0.77 &  0.84 &  0.92 &  0.98 &  0.91 &  0.94 &  0.49 &  0.92 &    1 &  682 &    7 & 2338 &  44 & 216 & 260 & 216 \\
coffeemachine &   0.8 &  0.75 &  0.83 &   0.8 &  0.95 &  0.97 &  0.94 &  0.97 &  0.72 &  0.61 &  0.78 &  0.72 &  999 &  996 & 3188 & 3152 & 320 & 320 & 320 & 320 \\
     desklamp &     1 &  0.94 &   0.8 &  0.87 &     1 &  0.91 &  0.84 &  0.99 &     1 &  0.97 &  0.79 &   0.8 &  254 &  255 & 1524 & 1521 &  12 &  56 & 244 & 244 \\
      desktop &   - &  0.96 &   - &  0.86 &   - &     1 &   - &     1 &   - &  0.93 &   - &  0.75 &  - &  184 &  - &  184 & - &  56 & - &  56 \\
       faucet &  0.85 &  0.86 &  0.92 &  0.92 &  0.84 &  0.85 &  0.98 &  0.96 &  0.89 &  0.92 &  0.88 &  0.89 &  921 & 1663 & 4759 & 8948 & 602 & 480 & 704 & 704 \\
    floorlamp &  0.58 &  0.86 &   0.8 &  0.88 &  0.83 &  0.75 &  0.92 &  0.98 &   0.5 &     1 &  0.75 &  0.83 &   88 &   68 &  318 &  272 &  44 &  12 &  62 &  62 \\
       laptop &   0.7 &  0.75 &  0.71 &  0.72 &  0.91 &  0.83 &  0.88 &  0.89 &  0.61 &  0.74 &  0.61 &  0.63 & 1545 & 1777 & 7170 & 8499 & 432 & 432 & 432 & 432 \\
    microwave &  0.86 &  0.81 &  0.85 &  0.89 &     1 &     1 &     1 &  0.99 &  0.76 &  0.72 &  0.74 &  0.81 & 1131 & 1124 & 3155 & 3177 & 252 & 252 & 252 & 252 \\
   showerhead &   - &     1 &   - &  0.84 &   - &     1 &   - &  0.88 &   - &     1 &   - &  0.89 &  - &   12 &  - &   48 & - &  46 & - &  94 \\
   television &  0.92 &  0.94 &  0.98 &  0.98 &  0.99 &  0.94 &     1 &     1 &  0.85 &  0.95 &  0.96 &  0.96 &  269 &  510 & 1104 & 1409 & 222 & 238 & 238 & 238 \\
      toaster &   0.6 &  0.81 &  0.71 &  0.81 &  0.86 &  0.98 &  0.99 &  0.98 &  0.59 &   0.7 &  0.58 &  0.71 &  713 & 1072 & 2180 & 3006 & 280 & 280 & 280 & 280 \\
       \hline\hline
 Weighted avg &  0.78 &  0.81 &   0.8 &  0.81 &   0.9 &  0.88 &  0.92 &  0.92 &  0.74 &   0.8 &  0.73 &  0.76 &    - &    - &    - &    - &   - &   - &   - &   - \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/toggle_metrics_learning.tex <==
\begin{table}[t]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lll|ll|ll|ll}
\toprule
& \multicolumn{2}{c|}{$Test$}  &  \multicolumn{2}{c|}{$Train$} &  \multicolumn{2}{c|}{$P$}&  \multicolumn{2}{c}{$R$}\\
 Object type &    \textsf{ND} &    \textsf{GTD} &  \textsf{ND} &    \textsf{GTD} &  \textsf{ND} &    \textsf{GTD} &   \textsf{ND} &   \textsf{GTD}\\
\midrule
       candle &       54 &         124 &        3 &         118 &          0.59 &        0.33 &       0.63 &         0.6 \\
    cellphone &      - &         216 &      - &         682 &           - &        0.84 &        - &        0.94 \\
coffeemachine &      320 &         320 &      999 &         996 &          0.95 &        0.97 &       0.72 &        0.61 \\
     desklamp &       12 &          56 &      254 &         255 &             1 &        0.91 &          1 &        0.97 \\
      desktop &      - &          56 &      - &         184 &           - &           1 &        - &        0.93 \\
       faucet &      602 &         480 &      921 &        1663 &          0.84 &        0.85 &       0.89 &        0.92 \\
    floorlamp &       44 &          12 &       88 &          68 &          0.83 &        0.75 &        0.5 &           1 \\
       laptop &      432 &         432 &     1545 &        1777 &          0.91 &        0.83 &       0.61 &        0.74 \\
    microwave &      252 &         252 &     1131 &        1124 &             1 &           1 &       0.76 &        0.72 \\
   showerhead &      - &          46 &      - &          12 &           - &           1 &        - &           1 \\
   television &      222 &         238 &      269 &         510 &          0.99 &        0.94 &       0.85 &        0.95 \\
      toaster &      280 &         280 &      713 &        1072 &          0.86 &        0.98 &       0.59 &         0.7 \\
      \hline\hline
 Weighted avg &        - &           - &       - &           - &           0.9 &        0.88 &       0.74 &         0.8 \\
\bottomrule
\end{tabular}
}
\caption{Size of the test set (columns 2-3) and generated training set (columns 4-5), precision (columns 6-7) and recall (columns 8-9) obtained by the neural network predicting the \textsc{toggle} property. The weighted average (last line) uses the number of test observations as weights.}
\label{tab:toggle_metrics_learning}
\end{table}

